NormGrad: Finding the Pixels that Matter for Training

The different families of saliency methods, either based on contrastive signals, closed-form formulas mixing gradients with activations or on perturbation masks, all focus on which parts of an image are responsible for the model's inference. In this paper, we are rather interested by the locations of an image that contribute to the model's training. First, we propose a principled attribution method that we extract from the summation formula used to compute the gradient of the weights for a 1x1 convolutional layer. The resulting formula is fast to compute and can used throughout the network, allowing us to efficiently produce fined-grained importance maps. We will show how to extend it in order to compute saliency maps at any targeted point within the network. Secondly, to make the attribution really specific to the training of the model, we introduce a meta-learning approach for saliency methods by considering an inner optimisation step within the loss. This way, we do not aim at identifying the parts of an image that contribute to the model's output but rather the locations that are responsible for the good training of the model on this image. Conversely, we also show that a similar meta-learning approach can be used to extract the adversarial locations which can lead to the degradation of the model.

==> fig-splash.tex <==
\begin{figure}\centering
\includegraphics[width=\linewidth]{figures/splash2_1}
\includegraphics[width=\linewidth]{figures/splash3_1}
\caption{Meta-learning can be used to determine training saliency - the pixels relevant for training a deep neural network - at different stages during learning. Left to right: training saliency at the beginning, middle, and end of learning to classify ImageNet images.}
\label{f:splash}
\end{figure}

==> figures/meta_procedure.tex <==

\begin{algorithm}
\caption{Meta-learning training saliency}    \label{f:meta_procedure}
\begin{algorithmic}[1]
\Require $\Phi_\theta$: randomly initialised network of depth $K$
\Require J: number of mask optimisation steps
\Require $\alpha$: $\mathcal{L}_{\text{area}}$ parameter
\Require $\mathcal{D} = (\mathcal{X}, \mathcal{Y}) $:  
\Statex $\mathcal{X} \in \mathbb{R}^{N \times H\times W\times 3}$, $\mathcal{Y} \in \{1,\dots,C\}^{N}$
\While{not done}
    \State $\Phi_\theta$ $\leftarrow$ train $\Phi_\theta$ on $\mathcal{D}$
    \For{$l \in [0, K), i \in [0, N)$}
        \State $\bx=\mathcal{X}_i, y=\mathcal{Y}_i$
        \State Split network at $l$:
        $\Phi_{\theta} = \Phi_{\theta}^{l-} \circ \Phi_{\theta}^{l+}$
        \State Initialize $\bbm = 0.5^{H\times W}$
        \For{$j \in [0,J)$}
            \State $\theta' \leftarrow \theta - \eta \nabla_\theta \ell(\Phi_{\theta}^{l+}(\bbm \otimes \Phi_{\theta}^{l-}(\bx)), y)$
            \State Compute $\mathcal{L}(\bbm) = - \ell(\Phi_{\theta'}(\bx),y)$ 
            \State \hspace{0.3cm} $+ \lambda_1 \|\bbm\|_{TV} + \lambda_2 \mathcal{L}_{\text{area}}(\bbm;a)$
            \State $\bbm \leftarrow \bbm - \eta \frac{d\mathcal{L}(\bbm)}{d\bbm}$
        \EndFor
        \State \textbf{yield} $\bbm$
    \EndFor
\EndWhile
\end{algorithmic}
\end{algorithm}



\begin{comment}
\Procedure{MyProcedure}{}
\State $\textit{stringlen} \gets \text{length of }\textit{string}$
\State $i \gets \textit{patlen}$
\BState \emph{top}:
\If {$i > \textit{stringlen}$} \Return false
\EndIf
\State $j \gets \textit{patlen}$
\BState \emph{loop}:
\If {$\textit{string}(i) = \textit{path}(j)$}
\State $j \gets j-1$.
\State $i \gets i-1$.
\State \textbf{goto} \emph{loop}.
\State \textbf{close};
\EndIf
\State $i \gets i+\max(\textit{delta}_1(\textit{string}(i)),\textit{delta}_2(j))$.
\State \textbf{goto} \emph{top}.
\EndProcedure
\end{comment}

==> intro.tex <==
\section{Introduction}\label{s:introduction}



The common wisdom is that deep neural networks require large training datasets, consisting of millions of images.
However, some researchers have questioned whether this assumption is valid. For instance, He et al.~\cite{he2018rethinking} has demonstrated that pre-training networks on large datasets such as ImageNet is not necessary to achieve good performance in much smaller datasets such as MS COCO. Similarly, Birodkar et al.~\cite{birodkar2019semantic} showed that there are notable numbers of redundant samples in ImageNet and CIFAR that can be removed without impacting validation performance. However, in general it remains unclear exactly what parts of a dataset are redundant.

\input{fig-splash}

Interest in demonstrating that neural networks can be effectively trained with smaller datasets is motivated by several reasons.
%The ability to maintain high validation performance with small datasets
First, this means reduced costs, both for training and data collection, which are common bottlenecks for deploying deep learning on new tasks~\cite{bach2017learning}.
Furthermore, distilling datasets is of importance in continual and life-long learning, where many approaches require maintaining a compressed store of data samples 
%that is optimized conjointly with non-stationary inputs, 
in order to alleviate catastrophic forgetting~\cite{shin2017continual, rolnick2018experience}.
Removing redundancy in data can significantly improve the scalability of such memory-based methods to the point that remembering all past data outright may become a feasible approach.
For instance, a back-of-the-envelope calculation suggests that by the time the human visual system is fully developed, a human may have ingested roughly 4 billion images.%
\footnote{
The development of vision in humans is usually largely completed by 4 years of age~\cite{braddick2011development}.
Assuming an image representation requiring 0.03 bits per pixels~\cite{wu18video}, 1MP images, 25fps, and a 12 hrs/day vigil, then by 4 years of age the toddler has seen roughly 50PB worth of visual data, or 4B images.
}
This is a large number, but already in the ballpark of trainable datasets~\cite{mahajan18exploring}, and likely to be significantly reduced by removing redundancy in the data.

Most of prior work on studying the redundancy of training data has focused on images as the basic unit of information that can be either retained or forgot~\cite{vodrahalli2018all, lapedriza2013all, angelova2005pruning}.
However, while humans can remember visual stimuli, they are well known to lack a perfect, photographic recollection of past events; instead, they compress information and selectively recall more \emph{memorable} patterns~\cite{schacter2012future}.
This suggests that not only are many training images redundant as whole, but it may suffice to recall only some essential portion of the image rather than a perfect copy of it.

In this paper, we refine this investigation and look at which~\emph{pixels} in an image are most responsible for contributing to learning a deep neural network on standard tasks such as image classification.
%First, we discuss the relationship between training saliency and inference saliency, and explain why considering the latter is not sufficient for understanding how neural networks train~(\cref{s:related}). 
We propose a meta-learning approach, in which training images are occluded by masks that are optimised to minimise task performance, thus revealing the regions on which training is highly dependent~(\cref{s:metamethod}).
This approach is principled, but it is also slow due to the need of performing double back-propagation.
Hence, we also develop a gradient-based approximation which is less principled, but much faster in practice~(\cref{s:gradmethod}).

We compare these two approaches and several baselines using a rigorous quantitative assessment protocol~(\cref{s:experiments}).
To assess the quality of each method, we use it to determine the set of highly salient training pixels within each image, delete the least salient pixels (e.g. 70\%), retrain a model from scratch on the reduced dataset, and assess the corresponding validation performance on unaltered images. The accuracy results show that our meta-learning approach is superior to gradient-based approximation for determining the relevant training pixels in the more challenging ImageNet experiments, whereas both are comparable for CIFAR-10. We find that a majority of pixels (70\%-80\%) can be discarded with a relatively modest impact on final performance (3.9\%-21.9\% drop), showing that it is possible to heavily reduce datasets to specific salient training regions whilst maintaining good task performance. 

Our training saliency procedures can be used for visualization by explicitly identifying which parts of an image play important roles at different stages of training a deep network~(\cref{f:splash}).
As discussed in~\cref{s:related} and ~\cref{s:gradmethod}, there are interesting similarities with inference saliency (attribution).
We explore this by comparing against popular attribution technique Grad-CAM~\cite{selvaraju17gradcam}, and find that models trained with masked datasets determined by our approach outperform those trained with those occluded by masks from Grad-CAM.
This is unsurprising as our methods are directly formulated for training saliency, and we believe our work is the first time this problem has been considered.

%This problem is similar to the \emph{attribution} task, where the goal is to identify which pixels are most responsible for the \emph{inference} performed by a neural network.
%Usually, attribution is solved by estimating a \emph{saliency map} ranking pixels by their importance in determining the network's output.
%Here, we instead look for which pixels are most responsible for \emph{learning} the model instead.
%Hence, our work can also be interpreted as a form of saliency referred to learning instead of inference.
%We believe this is the first time this problem has been considered.

%We evaluate our approach on a number of standard benchmarks, including CIFAR10, CIFAR100 and a reduced version of ImageNet (due to the computational cost).
%We show that we can discard a majority of the pixels from the training images with a relatively modest impact on the final model performance.
%This suggests that it is indeed possible to focus not only at retaining images as memories of the past, but to focus on specific content within these images, thus enabling greater compression and selectivity in the collection and storage of training data.




==> related.tex <==
\section{Related work}\label{s:related}

\paragraph{Inference saliency.}

Saliency can be defined as seeking the relevant parts of a dataset with respect to a task~\cite{dabkowski2017real}.
Note there is a difference between finding the pixels in an image that are salient for \emph{training}, and those that are salient for \emph{inference}.
The two are related notions, since any input pattern that is discriminated by a trained neural network has been learned in training; however, the reverse is not necessarily true.

%Thus, considering inference saliency is not sufficient for understanding how neural networks train.
Thus, considering inference saliency is insufficient if one seeks the data samples that are vital to network training.

Inference saliency, i.e.~finding the image parts that are relevant for decision making given a trained model, has been widely explored.
These methods generally produce pixel-wise masks per image as ours does.
A well-known approach is to compute the derivative of the task objective with respective to the input, and assume that high-gradient regions in the input correspond to salient regions~\cite{simonyan14deep}.
This has been extended by for example changing the ReLU derivatives~(Deconvnet~\cite{zeiler2014visualizing}, guided backprop~\cite{springenberg2014striving}) or averaging over randomly perturbed inputs~(SmoothGrad~\cite{smilkov2017smoothgrad}) to produce masks with reduced noise.
Many works have explored visualising saliency at intermediate levels within networks by combining weight values or gradients with activations, notably CAM~\cite{zhou2016learning}, Grad-CAM~\cite{selvaraju17gradcam}, Excitation Backprop~\cite{zhang2016excitation} and LRP~\cite{bach2015pixel}.


In response to the susceptibility of gradient-based saliency techniques to noise and artifacts~\cite{dabkowski2017real,fong17interpretable}, a number of works have sought to determine saliency by \emph{perturbing} the input and observing the change in output, thereby grounding the saliency mask in a known set of explicitly interpretable image manipulations.
\cite{zeiler2014visualizing} and~\cite{Petsiuk2018rise} generate saliency masks by weighting input occlusion patterns by the induced changes in model output.
\cite{fong17interpretable} optimises for masks that maximally affect a model's output, using the total-variation norm and upsampling to restrict mask expressiveness;
\cite{dabkowski2017real} builds on this by learning a model for predicting masks that maximally affects output.
Perturbation-induced output response has also been used to perform object localisation~\cite{singh2017hide, wei2017object, wang2017fast}.

\paragraph{Training saliency and dataset distillation.}

The use of large amounts of labelled training data is a well-known limitation of deep networks, leading to interest in demonstrating that neural networks can be effectively trained with smaller datasets.
Recently, it was shown that pre-training on large datasets such ImageNet is not necessary for obtaining state-of-the-art performance in much smaller datasets such as MS COCO~\cite{he2018rethinking}.
There are two general approaches for reducing datasets: compressing image datasets such that they can be reconstructed faithfully, and compressing image datasets such that training on them leads to validation performance that is comparable to using the original full version.

The latter includes our work.
Of relevance is dataset distillation~\cite{wang2018dataset}, which compresses an entire dataset into very few (e.g.~10) synthetic images.
The produced images are not natural looking, meaning the method is effectively a network weight compression technique.
Retraining requires careful consideration of initialisation, and due to the tangled nature of the resulting synthetic dataset, it is unclear how new images or classes could be added, or what was salient in the original dataset.


Many methods for reducing datasets by eliminating individual images (and thus maintaining dataset realism and disjointness) have been proposed~\cite{vodrahalli2018all, angelova2005pruning, felzenszwalb2010object, lapedriza2013all}.
Core-sets have been used to seek dataset subsets that allow models to perform as well as when the full dataset is used~\cite{sener2017active, bachem2017practical, har2007smaller, tsang2005core}.
Influence functions~\cite{koh17understanding} have been used to estimate the effect of removing or perturbing an input image on the network parameters, allowing for input images to be ranked by their influence on specific image classes.
Most recently~\cite{birodkar2019semantic} used agglomerative clustering to discover redundancies, and found that at least 10\% of the images in popular datasets CIFAR10 and ImageNet are removable without any impact on validation accuracy.
Unlike our work, these methods have focused on training saliency as coarsely curating whole images, rather than at the higher granularity of pixels within images.


At a high level, dataset reduction is related to knowledge distillation via attention.
It has been shown that training networks to replicate the spatial attention behaviour of more optimised networks improves their overall performance~\cite{zagoruyko2016paying}.
In this case spatial attention maps are used to transfer attention patterns between networks rather than reduce the dataset.

There is, of course, an extensive field focused on image compression for high-fidelity reconstruction, not least codecs~\cite{wallace1992jpeg} and image generation with autoencoders and adversarial methods~\cite{dosovitskiy2016generating, ledig2017photo}.
Of particular relevance to our work are approaches that compress images with importance-weighted codes~\cite{li2018learning, prakash2017semantic}, with salient pixels prioritised in the compressed code.

\paragraph{Life-long learning and catastrophic forgetting.}

Recently, a distinct subset of knowledge distillation relating to life-long learning has received significant attention.
Specifically, storing previously seen dataset samples and training conjointly with non-stationary inputs alleviates catastrophic forgetting arising from the latter~\cite{shin2017continual}.
A variety of different sample compression have been explored, ranging from learning exemplars per class~\cite{rebuffi2017icarl}, to training generators to functionally produce samples representative of the full observed distribution~\cite{shin2017continual, kemker2017fearnet, ramapuram2017lifelong, draelos2017neurogenesis}.
Rehearsing stored data from experience replay buffers is a common practice in reinforcement learning~\cite{mnih2013playing}, and~\cite{rolnick2018experience} has explored repurposing the buffer as an aid against catastrophic forgetting by treating it as a distilled store of previously seen samples with random selection.
A study on selective replay~\cite{isele2018selective} found that coverage maximisation and distribution matching with the original data were suitable metrics for reducing storage buffer size whilst mitigating catastrophic forgetting.
These objectives are analogous to ours, which is to reduce the pixels whilst preserving the salient parts of each image and thus maintaining the original class distribution.







==> theory.tex <==
% -----------------------------------------------------------------------------
\section{Theory of feature frames}
% -----------------------------------------------------------------------------

Let $\bbf_0 \subset \mathbf{R}^2$ be a \emph{canonical frame}, such as a point, a circle, a line, or a square. Let $G$ be a group of transformations $g:\mathbb{R}^2\rightarrow\mathbb{R}^2$, such as translations, dilations, rigid motions or affinities. The pair $(G,\bbf_0)$ \emph{generates} the space of feature frames given by
$$
\mathcal{F} = G \bbf_0 = \{ g \bbf_0 : g \in G \}.
$$
For example, if $\bbf_0 = \{0\}$ is a point and $G=T(2)$ are the two dimensional translations, then $\mathcal{F}=\mathbb{R}^2$ are all possible points. If $\bbf_0$ is the unit circle centred at the origin and $G=E(2)$ are the two dimensional Euclidean transformations, then $\mathcal{F}$ are all possible circles.

By construction, we can apply any transformation to frames:
\begin{proposition}
  The set $\mathcal{F}$ is closed under the action of $G$, in the sense that $G\mathcal{F} = \mathcal{F}$.
\end{proposition}

% -----------------------------------------------------------------------------
\subsection{Symmetries of frames}
% -----------------------------------------------------------------------------

Each canonical frame $\bbf_0$ has a corresponding set of \emph{symmetries}, which are the transformations that leave $\bbf_0$ unchanged:
$$
  S = \{ s \in G : \bbf_0 = s \bbf_0 \}.
$$
The symmetries $S$ are a subgroup of $G$, called the \emph{symmetry group} of $\bbf_0$:
\begin{proposition}
The set of symmetries $S$ of a frame $\bbf_0 \subset \mathbb{R}^2$ is a subgroup of $G$.
\end{proposition}
\begin{proof}
It suffices to show that $S$ is closed under the group operation (composition of transformations) and group inverse. In fact, if $s_1,s_2\in S$, then $\bbf_0 = s_1\bbf_0 =s_2\bbf_0$, $\bbf_0 = s_1(s_2(\bbf_0))$, so that $s_1s_2\in S$. Furthermore, if $s \in S$, then $\bbf_0 = s\bbf_0$, so that $s^{-1}\bbf_0 = \bbf_0$, and $s^{-1}\in S$.
\end{proof}
For example, if $\bbf_0 = \{0\}$ is the origin and $G = E(2)$ the 2D Euclidean transformations, then the symmetry group are the 2D rotations $S = SO(2)$. If, on the other hand, $G= A(2)$ is the group of 2D affinities, then $S = GL(2)$ is the group of 2D linear transformations. Note that in this examples it is important that $\bbf_0$ is the origin as choosing another point would result in an analogous but less natural symmetry group. This is clarified in full generality next.

Consider a frame $\bbf = g\bbf_0$. The symmetries of $\bbf$ are the conjugate of the ones of $\bbf_0$, in the sense that:
\begin{proposition}\label{p:sym-conj}
If $\bbf = g\bbf_0$ and $S$ is the symmetry group of $\bbf_0$, then the symmetry group of $\bbf$ is the conjugate group $gSg^{-1}$.
\end{proposition}
\begin{proof}
Let $S'$ be the group of symmetries of $\bbf$. First, we show that $gSg^{-1}\subset S'$; to do so, we must show that, for any $s \in S$, the transformation $g s g^{-1}$ is a symmetry of $\bbf$. In fact: $g s g^{-1}\bbf = g s \bbf_0 = g \bbf_0 = \bbf$. Next, we show that $S' \subset gSg^{-1}$. To this end, let $s'$ be any symmetry of $\bbf$, so that $s' \bbf = \bbf$, $s' g \bbf_0 = g \bbf_0$, and $g^{-1}s' g \bbf_0 = \bbf_0$. The latter result means that $g^{-1}s'g \in S$, so that $s' \in gSg^{-1}$.
\end{proof}
\begin{corollary}
Let $g,t\in G$ be two transformations that generate the same frame, i.e.\ $\bbf = g \bbf_0 = g' \bbf_0$, and let $S$ be the symmetry group of $\bbf_0$. Then $gSg^{-1} =tSt^{-1}$.
\end{corollary}
\begin{proof}
Since the symmetry group of any frame is unique, the expression for the symmetry group of $\bbf$ found in~\cref{p:sym-conj} must not depend on $g$.
\end{proof}

% -----------------------------------------------------------------------------
\subsection{Frames as geometric references}
% -----------------------------------------------------------------------------

Frames allow to fix transformations up to symmetries. First, we show that a frame $\bbf = g \bbf_0$ can be obtained from the canonical frame $\bbf_0$ by an equivalence class of transformations $g$; more precisely, if $g$ is a transformation solving this equation, then all the others can be written as the \emph{(left) coset} $gS = \{gs : s \in S \}$.

Recall that the cosets of a subgroup $S \subset G$ induce an equivalence relation $\equiv_S$ and a corresponding partition $G/S$ of the group $G$ (if $S$ is a normal subgroup, then $G/S$ has a group structure --- the quotient group) such that two transformations $g \equiv_S g'$ are equivalent if, and only if, they belong to the same coset.

There is a natural correspondence between cosets and frames:
\begin{proposition}\label{p:framecosets}
Any two transformations $g',g\in G$ generate the same frame if, and only if, they belong to the same coset, i.e.
$$
\forall g,g'\in G:\quad g \bbf_0 = g' \bbf_0 \quad\Leftrightarrow\quad g \equiv_S g'.
$$
\end{proposition}
\begin{proof}
If $g \equiv_S g'$, there exists a symmetry $s\in S$ such that $g' = gs$ and $g' \bbf_0  = gs \bbf_0 = g \bbf_0$. If $g' \bbf_0 = g \bbf_0$, then $g^{-1}g' \bbf_0 = \bbf_0$, $g^{-1}g' \in S$, and $g' \in gS$.
\end{proof}

\begin{proposition}
The map $G/S \rightarrow \mathcal{F}$ obtained by mapping each coset $gS \in G/S$ to the frame $\bbf = g \bbf_0$ is a bijection between cosets and frames.
\end{proposition}
\begin{proof}
First, note that the rule given defines a proper function. This is because, while the same coset can be written as $gS$ for different transformations $g$, from \cref{p:framecosets} all such choices results in the same frame $g\bbf_0$. Next,  the map is surjective because any transformation $g$ is contained in a coset, so that the codomain is the whole of $\mathcal{F}$. Finally, the map is injective because, if two cosets $gS, g'S$ map to the same frame $g\bbf_0 =g'\bbf_0$, then for \cref{p:framecosets} they must be the same coset.
\end{proof}

Next, we consider the transformations identified by a pair of frames.
\begin{proposition}
Let $\bbf_0$ be the canonical frame and $S$ its symmetry group. Given any two frames $(\bbf_1,\bbf_2)$, the solutions of the equation $\bbf_2 = g \bbf_1$ are given by $g_2 S g_1^{-1}$ where $g_i,i=1,2$ are any two transformations such that $\bbf_i = g_i \bbf_0$.
\end{proposition}
\begin{proof} First, we show that, for any choice of $g_i:\bbf_i = g_i \bbf_0$, then any element of $g_2 S g_1^{-1}$ is a solution. To show this, pick any $s \in S$ and note that
$
(g_2 s g_1^{-1}) \bbf_1 = g_2 s \bbf_0 = g_2 \bbf_0 = \bbf_2.
$
Next, we show that, for any fixed choice of $g_i: \bbf_i = g_i \bbf_0$, any solution $g$ can be written as $g_2 s g_1^{-1}$ for a suitable $s \in S$:
$$
\begin{aligned}
\bbf_2 = g \bbf_1
&\quad\Rightarrow\quad
g_2\bbf_0 = g g_1 \bbf_0
\\
&\quad\Rightarrow\quad
\bbf_0 = (g_2)^{-1} g g_1 \bbf_0
\\
&\quad\Rightarrow\quad
(g_2)^{-1} g g_1 \in S.
\end{aligned}
$$
If we set $s = (g_2)^{-1} g g_1$, then
$
g_2 s g_1^{-1}
= 
g_2(g_2)^{-1} g g_1g_1^{-1}
=
g
$
as needed.
\end{proof}

% -----------------------------------------------------------------------------
\subsection{Representative and transversals}
% -----------------------------------------------------------------------------

Our goal is to represent frames $\bbf$ by means of transformations $G$. From the previous sections, it is clear that, if the canonical frame has non-trivial symmetries, then any frame $\bbf = g \bbf_0$ is generated by \emph{several different transformations} $g$. There are two possible way forward. The first one is to still use all transformations in $G$ but to account for their equivalence $\equiv_S$ in the calculations as needed. The second one is to pick a \emph{single representative transformation $r$} in each equivalence class $G/S$ and use $r$ to index frames. Here we investigate both options.

Formally, a \emph{(left) transversal $R$} of the subgroup $S\subset G$ is a subset $R \subset G$ that intersects each (left) coset exactly once:
$$
\forall g \in G : \quad
| R \cap g S | = 1.
$$
Since the cosets form a partition of $G$, the existence of such an $R$ is guaranteed by the axiom of choice.
\begin{proposition}
Given a subgroup $S$ and a corresponding transversal $R$, all transformations $g\in G$ have a unique decomposition $g = rs, r \in R, s\in S$. Furthermore, $G = RS$ is the product of the transversal and the subgroup.
\end{proposition}
\begin{proof}
Suppose that $g = rs = r's'$ are two decompositions where $s,s'\in S$. Then $r = gs^{-1}$ and $r' = g(s')^{-1}$ mean that $r$ and $r'$ are in the same coset. Since the transversal has a unique intersection with each coset, one must have $r=r'$, and so $s=s'$.
\end{proof}

Since there is a bijective correspondence between $R$ and $G/S$ and between $G/S$ and $\mathcal{F}$, then $R$ and $\mathcal{F}$ are also in bijective correspondence. This means that frames can be identified with representative transformations. 

Next, we explore the advantages of using either the equivalence classes or the representatives in calculations. Our main goal is to write the \emph{equivariance constraint} in terms of transformations. We start by stating it in terms of frames. To this end, let $\tilde \phi : \mathcal{X} \rightarrow \mathcal{F}$ be a map from images to frames. The map is equivariant with $g$ if
$$
    \forall g \in G:\quad \tilde \phi(g \bx) = g \tilde \phi(\bx).
$$
The larger the symmetry group of the canonical frame, the weaker the constraint (and the least amount of work is required from the detector function $\tilde \phi$). Since working with frames (which are actual geometric shapes) is cumbersome, we prefer to represent them using transformations instead. Since frames are generated by the group $G$, the idea is to replace $\tilde \phi:\mathcal{X} \rightarrow \mathcal{F}$ with $\phi: \mathcal{X} \rightarrow G$. Since, however, there are several transformations that correspond to the same frame, this must be done carefully. One way is to consider the equivalence relation $\equiv_S$ between transformations:
$$
    \forall g \in G:\quad \phi(g \bx) \equiv_S g \phi(\bx)
$$
which can be written more explicitly as:
\begin{equation}\label{e:cov2}
    \forall g \in G: \exists s \in S : \phi(g \bx) s = g \phi(\bx).
\end{equation}
The main disadvantage of this formulation is that the existence of $s$ must be checked every time the constraint is asserted.

A different option is to use representatives, so that each frame is associated with a unique transformation $\phi : \mathcal{X} \rightarrow R$. The problem with this approach is that the representatives $R$ are in general \emph{not} closed under the action of $g$. Thus, we need to introduce the function $\pi_R : G \rightarrow R$ which project each transformation $g$ to the representative $r$ of the corresponding coset $gS$. Then the constraint can be written as
$$
    \forall g \in G: \phi(g \bx) = \pi_R\left[ g \phi(\bx) \right].
$$
Thus we see that using representatives may not necessarily simplify calculations.

Sometimes, it is possible to choose $R$ so that simplifications ensue.
In particular, assume that the transversal $R$ forms a \emph{normal subgroup} of $G$ (normality means being invariant to conjugation, i.e.\ $r \in R \Rightarrow g r g^{-1} \in R$). In this case, we can show that the choice of $s$ in \cref{e:cov2} does \emph{not} depend on $\phi$ and can be carried out beforehand based on $g$ alone.

\begin{proposition}
Let $S \subset G$ be a subgroup of $G$ and let $R$ be a transversal of $S$ which is also a normal subgroup $R \triangleleft G$. Consider two decompositions
$$
r_2 s = g r_1,
\quad
r_2' s' = g r_1'
$$
where $g \in G$, $r_1,r_2,r_1',r_2' \in R$, and $s,s'\in S$. It must be $s=s'$.
\end{proposition}
\begin{proof} We have
$s = r_2^{-1} g r_1$ and
$s' = (r_2')^{-1} g r_1'$. Hence
$$
s(s')^{-1}
=
(r_2^{-1} g r_1)((r_1')^{-1} g^{-1} r_2')
=
r_2^{-1} g r g^{-1} r_2'
$$
where $r = r_1 r_1'^{-1} \in R$ since $R$ is a group. Since $R$ is normal $r' =g r g^{-1} \in R$ as well. Hence
$$
S \ni s(s')^{-1} = r_2^{-1} r' r_2' \in R.
$$
Since $S,R$ are subgroups, they must contain the identity $1$ and $1 \in S \cap R$. Since $R$ is transversal, this must also be the sole intersection. We conclude that $s(s')^{-1} =1$, and so $s = s'$.
\end{proof}

Based on this proposition, we can get another variant of constraint~\eqref{e:cov2}:
\begin{equation}\label{e:cov3}
    \forall g \in G: \phi(g \bx) s_g = g \phi(\bx).
\end{equation}
where the choice of $s_g \in S$ depends on $g$ only.

\subsection{Other results which may nor may not be useful}

\begin{proposition}
If the left transversal $R$ of a subgroup $S\subset G$ is  a subgroup of $R$, then it is also a right transversal.
\end{proposition}
\begin{proof}
We need to show that $|R \cap S g| = 1$ for all $g \in G$. First, we show that if there is an intersection between $R$ and the right coset $Sg$, then this is unique. To show this, consider two elements $r,r' \in (R \cap Sg)$. They can be written as $r = sg$ and $r' = s'g$ for some $s,s' \in S$. Since $R$ is a group, we have $R \ni r'r^{-1} = s'gg^{-1}s^{-1} = s's^{-1} \in S$. Since $R$ is a left transversal, $R \cap S = 1$, $s's^{-1}=1$, $s=s'$ and $r = sg = s'g =r'$. Hence then intersection $R \cap S g$ contains at most one element.

Next, we show that the intersection is not empty. In order to do so, we must show that, for any $g\in G$, we can find an element $s\in S$ such that $sg \in R$. Since $R$ is a left transversal, this means that there is an $s'$ such that $g^{-1}s' \in R$ (because $R$ intersects the left coset $g^{-1} S$). Since $R$ is a group, taking the inverse shows that $(s')^{-1}g \in R$ as well. Since $S$ is a group as well, $(s')^{-1}\in S$ as need.
\end{proof}

